Optimized Coverage Planning for UV Surface Disinfection

UV radiation has been used as a disinfection strategy to deactivate a wide range of pathogens, but existing irradiation strategies do not ensure sufficient exposure of all environmental surfaces and/or require long disinfection times. We present a near-optimal coverage planner for mobile UV disinfection robots. The formulation optimizes the irradiation time efficiency, while ensuring that a sufficient dosage of radiation is received by each surface. The trajectory and dosage plan are optimized taking collision and light occlusion constraints into account. We propose a two-stage scheme to approximate the solution of the induced NP-hard optimization, and, for efficiency, perform key irradiance and occlusion calculations on a GPU. Empirical results show that our technique achieves more coverage for the same exposure time as strategies for existing UV robots, can be used to compare UV robot designs, and produces near-optimal plans. This is an extended version of the paper originally contributed to ICRA2021.

==> figs/results.tex <==
\section{\label{sec:results}Experiments \& Results}

\subsection{2.5D experiments}

\subsubsection{Comparison against single point}

We first evaluated our performance in a baseline case of a 5x5 empty room - comparing single-point (at the centroid) disinfection strategies with our proposed solution in terms of disinfection efficiency (i.e. how long it took until complete disinfection was achieved).

We randomly generated 25 2.5D worlds with a number of geometric obstacles ranging from 7 to 19 (mean 13.7) and evaluated single-point disinfection strategies against our proposed solution in terms of maximum achievable coverage (i.e, what fraction of the surface area received at least $\mu_{min}$ fluence) and time until full disinfection (how much dwell time is needed to guarantee that all visible surfaces get $\mu_{min}$ fluence).

The single point disinfection strategy consisted in placing the disinfection light at the point that had maximum coverage over the obstacle space and allowing it to irradiate the surfaces for as long as necessary to fully disinfect its visible surfaces. In this scenario, we discretized the 2D space with a grid of 25cm when choosing candidate vantage configurations for the robot.

The results of this experiment are seen in \prettyref{fig: Single Point 2D Comparisons}, our proposed method consistently disinfected 100\% of the environment, whereas the optimal single vantage point could only disinfect, on average, 35\% of the environment's area, a difference clearly seen in \prettyref{fig: single point vs multi-point 2.5D}.  

\begin{figure}[htbp] % "[t!]" placement specifier just for this example
    \centering
    \includegraphics[width=0.9\linewidth]{figs/Single Point 2D comparisons.pdf}
    \caption{Comparison between our method and single point strategy} \label{fig: Single Point 2D Comparisons}
\end{figure}

\begin{figure}[htbp] % "[t!]" placement specifier just for this example
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/Example of Optimally Placed Single point Disinfection.pdf}
    \caption{Single Point Disinfection}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
    \includegraphics[width=\linewidth]{figs/Ours 2D disinfection .pdf}
    \caption{Multipoint Disinfection} 
    \end{subfigure}
    \caption{Same room disinfected by the best single point and by our method, where the trajectory is represented as a red line and each surface is colored according to the fluence it received.}
    \label{fig: single point vs multi-point 2.5D}
\end{figure}

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \centering
% \includegraphics[width=0.49\linewidth]{figs/Single Point 2D comparisons.pdf}
% \includegraphics[width=0.49\linewidth]{figs/towerbot 30 mins.png}
% \caption{\label{fig: single point 3D disnfection} We compared stationary (left) and moving (right) light mounting strategy, where surfaces are painted on a spectrum from red (0 fluence received) to green (received at least $280J/m^2$ of fluence). Left: A stationary light source leaves much of an environment still infected (in red), even after $30$ minutes. Right: A mobile robot given the same time budget and following our optimally computed trajectory (in orange) covers the space much better - as evidenced by corners and sides }
% \vspace{-10px}
% \end{figure}



\subsubsection{Comparison against MILP formulation}

On a subset of those rooms, we evaluated the performance of our proposed sequential approach when compared to the optimal MILP formulation in terms of time for total disinfection and path length, using gridding of 50 cm to enable the feasibility of the MILP. We additionally assumed a mean velocity of 0.5 m/s of the robot when computing the solutions.

\prettyref{fig: MILP VS LP} shows that we observed little difference between the total disinfection times obtained via the MILP and our sequential formulation as evidenced by the mean normalized dwell times and disinfection times. This is likely due to the fact that the dwell time in both cases represented on average 90\% of total disinfection time and, hence, not optimizing for moving time does not heavily affect the optimality of our solution. Most crucially, we note that the sequential approach yields results over 30 times faster than the optimal MILP solution - even in such simplified settings.

% When compared to the optimal MILP formulation of the trajectory optimization problem, our proposed solution,at least for the gridding resolutions used, did not manifest a remarked loss of optimality, taking, on average, only 2.7\% longer to completely disinfect the 2.5D environments. In addition, our initial hypothesis that the majority of the disinfection time would be dwell time was confirmed since, in both algorithms, the time to move between the vantage points represented fewer than 10\% of the total disinfection time. In addition, our method was remarkably faster than the true optimal solution, which took, on average, 31.5 times longer to compute . \textcolor{red}{missing measure of spread - asked Ramya for data}

\begin{figure}[htbp] % "[t!]" placement specifier just for this example
    \centering
    \includegraphics[width=0.9\linewidth]{figs/MILP and LP comparisons.pdf}
    \caption{Comparison between our sequential approach and the optimal MILP. Times normalized w.r.t. LP+TSP times for contrast} \label{fig: MILP VS LP}
\end{figure}


\subsection{3D experiments}

Our 3D tests were performed in a modified version of a hospital infirmary\footnote{https://grabcad.com/library/hospital-ward-2-2}, which was modified for cohesion and scaling and had its mesh simplified to 60k triangles using MeshLab's \cite{cignoni2008meshlab} quadric edge collapse decimation to speed up computations. The gridding resolution distance, $\rho$ was 0.25m. Our experiments consisted of generating disinfection plans for Floatbot, Armbot, and Towerbot under a strict irradiation time limit of 30 minutes, as well as under a 100-hour time budget to the evaluate asymptotic disinfection performance of each design. We additionally evaluated placing Towerbot in the centroid of the room for the prescribed time budget to mimic the static status-quo.

% We then compared the total disinfection time of these 4 strategies: 
% \begin{itemize}
%     \item Executing an optimal disinfection plan for Floatbot
%     \item Executing an optimal disinfection plan for Armbot;
%     \item Executing an optimal disinfection plan for Towerbot
%     \item Placing Towerbot at the centroid of the room for as long as necessary to mimic the single-point status-quo.
% \end{itemize}

% We additionally performed the same experiments under a time constraint of 30 minutes in order to represent each strategy's efficiency under a strict time budget. 

\prettyref{fig: Robot Design Comparisons} illustrates that, as expected, robots with more degrees of freedom, like Armbot and Floatbot, disinfect more of the area, specially under tight time budgets and that, in accordance to \cite{Lindblad2019Ultraviolet-CNeeded}, the status-quo of static disinfection for tower-based roots fails to cover much of the surface, which is illustrated well in \prettyref{fig: single point 3D disnfection}. We note, however, that asymptotic performance is nearly identical among all mobile solutions.

Note, however, that the disinfection efficiency comes with tradeoff in total distance travelled, since Towerbot has the smallest trajectory length of all mobile solutions, whereas Armbot has the longest. 

This is likely due to two factors. First, distances in higher dimensions tend to be higher (3D vs 2D) and second, motion planning for Armbot involves many steps that are prone to suboptimality, such as vantage configuration selection given a desired lamp position and high-dimensional multi-query path planning, which is an active research area. Floatbot's trajectory length is a trivial lower bound to the Armbot's length. Jointly optimizing vantage configurations alongside a tour to minimize trajectory length is left to future research. 

Finally,\prettyref{fig:Smart 3D disnfection} shows a time-lapse of Armbot's disinfection trajectory.
% by Armbot  , where the disinfection trajectory of the UV lamp is highlighted in orange and the disinfection status of the room is color coded on a spectrum from red (0 fluence received) to solid green (received at least $\mu_{min} = 280 J/m^2$. 

\begin{figure}[htbp] % "[t!]" placement specifier just for this example
    \centering
    \includegraphics[width=0.95\linewidth]{figs/Robot Design Comparisons.pdf}
    \caption{Performance of robot designs disinfecting an infirmary} \label{fig: Robot Design Comparisons}
\end{figure}


% \begin{table}[htbp]
% \centering
% \begin{tabular}{ |l||c|c|c|c| } 

%  \hline \hline
%  \textbf{Method} & \textbf{Completion}  & \textbf{Coverage-1} & \textbf{Coverage-2}\\ & \textbf{time} & & \\
%  \hline
%  \textbf{Single} &  & & \\ 
%  \hline
%  \textbf{Towerbot} & 83.6 & & \\ 
%  \hline
%  \textbf{Ideal} & & & \\
%  \hline
%  \textbf{Armbot} & & & \\
%  \hline
% \end{tabular}
% \caption{Summary of 3D disinfection Experiments}
% \label{tab:3D experimental results}

% \end{table}

% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/2D example scene.pdf}
%     \caption{Example of the optimal 2D disinfection path on 2.5D scene} \label{fig: Example 2D trajectory}
% \end{figure}


    
%     \caption{Example of 2.5D disinfection of an empty square room. Vantage points are color-coded by the dwell time, and surface points are color-coded by the radiant exposure.  The single-point method underexposes the corners, so it takes 194\% more time than our method. } \label{fig: Empty Room disinfection}
%     \end{figure}


% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\linewidth]{figs/Complex Room disinfection Single.pdf}
%     \caption{Single Point Disinfection}
%     \end{subfigure}\hspace*{\fill}
%     \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\linewidth]{figs/Complex Room disinfection Multi.pdf}
%     \caption{Multipoint Disinfection} 
%     \end{subfigure}

    
%     \caption{Example of 2.5D disinfection of a room with randomly-generated obstacles. Both approaches were given the same time budget used by the multi-point disinfection to irradiate the room (400\,s). The single-point method only disinfects 20\% of the surfaces while our method disinfects the whole room.} \label{fig:2.5D disinfection of rooms}
%     \end{figure}
    
% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/single_tower_disinfection.png}
%     \caption{A stationary light source does not disinfect of the environment of Fig.~\ref{fig:Smart 3D disnfection} under the same 30 minutes budget nearly as well} \label{fig: single point 3D disnfection}
% \end{figure}


% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/histogram of time fractions.png}
%     \caption{Histogram of the fraction of time taken by movement during the disinfection of a set of 21 randomly generated 2.5D rooms} \label{fig: histogram of times}
% \end{figure}

% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/LP VS MILP.png}
%     \caption{Histogram of the extra time taken by our sequential approach when compared to the optimal solution} \label{fig: histogram of suboptimality}
% \end{figure}


\begin{figure*}[h!] % "[t!]" placement specifier just for this example
\setlength{\tabcolsep}{0.2px}
\begin{tabular}{cccc}
\includegraphics[width=.24\linewidth]{figs/a}
\put(-110,-10){\small{Disinfection at 7.5 minutes}} &
\includegraphics[width=.24\linewidth]{figs/Hospital CAD 50.png}
\put(-110,-10){\small{Disinfection at 15 minutes}} &
\includegraphics[width=.24\linewidth]{figs/Hospital CAD 75.png}
\put(-110,-10){\small{Disinfection at 22.5 minutes}} &
\includegraphics[width=.24\linewidth]{figs/Hospital CAD 100.png}
\put(-110,-10){\small{Disinfection at 30 minutes}} 
\end{tabular}
\caption{Demonstration of optimized disinfection of a hospital room CAD model, with a time budget of 30 minutes. Red indicates no disinfection, green indicates complete disinfection. The light's path is shown in orange and visited dwell points are shown in yellow, while unvisited ones are shown in black} \label{fig:Smart 3D disnfection}
\end{figure*}

==> results_old.tex <==
\section{\label{sec:results}Experiments \& Results}

\subsection{2.5D experiments}

\subsubsection{Comparison against single point}

We first evaluated our performance in a baseline case of a 5x5 empty room - comparing single-point (at the centroid) disinfection strategies with our proposed solution in terms of disinfection efficiency (i.e. how long it took until complete disinfection was achieved).

We randomly generated 25 2.5D worlds with a number of geometric obstacles ranging from 7 to 19 (mean 13.7) and evaluated single-point disinfection strategies against our proposed solution in terms of maximum achievable coverage (i.e, what fraction of the surface area received at least $\mu_{min}$ fluence) and time until full disinfection (how much dwell time is needed to guarantee that all visible surfaces get $\mu_{min}$ fluence).

The single point disinfection strategy consisted in placing the disinfection light at the point that had maximum coverage over the obstacle space and allowing it to irradiate the surfaces for as long as necessary to fully disinfect its visible surfaces. In this scenario, we discretized the 2D space with a grid of 25cm when choosing candidate vantage configurations for the robot.

The results of this experiment are seen in \prettyref{fig: Single Point 2D Comparisons}, our proposed method consistently disinfected 100\% of the environment, whereas the optimal single vantage point could only disinfect, on average, 35\% of the environment's area, a difference clearly seen in \prettyref{fig: single point vs multi-point 2.5D}.  

\begin{figure}[htbp] % "[t!]" placement specifier just for this example
    \centering
    \includegraphics[width=0.9\linewidth]{figs/Single Point 2D comparisons.pdf}
    \caption{Comparison between our method and single point strategy} \label{fig: Single Point 2D Comparisons}
\end{figure}

\begin{figure}[htbp] % "[t!]" placement specifier just for this example
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/Example of Optimally Placed Single point Disinfection.pdf}
    \caption{Single Point Disinfection}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
    \includegraphics[width=\linewidth]{figs/Ours 2D disinfection .pdf}
    \caption{Multipoint Disinfection} 
    \end{subfigure}
    \caption{Same room disinfected by the best single point and by our method, where the trajectory is represented as a red line and each surface is colored according to the fluence it received.}
    \label{fig: single point vs multi-point 2.5D}
\end{figure}

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \centering
% \includegraphics[width=0.49\linewidth]{figs/Single Point 2D comparisons.pdf}
% \includegraphics[width=0.49\linewidth]{figs/towerbot 30 mins.png}
% \caption{\label{fig: single point 3D disnfection} We compared stationary (left) and moving (right) light mounting strategy, where surfaces are painted on a spectrum from red (0 fluence received) to green (received at least $280J/m^2$ of fluence). Left: A stationary light source leaves much of an environment still infected (in red), even after $30$ minutes. Right: A mobile robot given the same time budget and following our optimally computed trajectory (in orange) covers the space much better - as evidenced by corners and sides }
% \vspace{-10px}
% \end{figure}



\subsubsection{Comparison against MILP formulation}

On a subset of those rooms, we evaluated the performance of our proposed sequential approach when compared to the optimal MILP formulation in terms of time for total disinfection and path length, using gridding of 50 cm to enable the feasibility of the MILP. We additionally assumed a mean velocity of 0.5 m/s of the robot when computing the solutions.

\prettyref{fig: MILP VS LP} shows that we observed little difference between the total disinfection times obtained via the MILP and our sequential formulation as evidenced by the mean normalized dwell times and disinfection times. This is likely due to the fact that the dwell time in both cases represented on average 90\% of total disinfection time and, hence, not optimizing for moving time does not heavily affect the optimality of our solution. Most crucially, we note that the sequential approach yields results over 30 times faster than the optimal MILP solution - even in such simplified settings.

% When compared to the optimal MILP formulation of the trajectory optimization problem, our proposed solution,at least for the gridding resolutions used, did not manifest a remarked loss of optimality, taking, on average, only 2.7\% longer to completely disinfect the 2.5D environments. In addition, our initial hypothesis that the majority of the disinfection time would be dwell time was confirmed since, in both algorithms, the time to move between the vantage points represented fewer than 10\% of the total disinfection time. In addition, our method was remarkably faster than the true optimal solution, which took, on average, 31.5 times longer to compute . \textcolor{red}{missing measure of spread - asked Ramya for data}

\begin{figure}[htbp] % "[t!]" placement specifier just for this example
    \centering
    \includegraphics[width=0.9\linewidth]{figs/MILP and LP comparisons.pdf}
    \caption{Comparison between our sequential approach and the optimal MILP. Times normalized w.r.t. LP+TSP times for contrast} \label{fig: MILP VS LP}
\end{figure}


\subsection{3D experiments}

Our 3D tests were performed in a modified version of a hospital infirmary\footnote{https://grabcad.com/library/hospital-ward-2-2}, which was modified for cohesion and scaling and had its mesh simplified to 60k triangles using MeshLab's \cite{cignoni2008meshlab} quadric edge collapse decimation to speed up computations. The gridding resolution distance, $\rho$ was 0.25m. Our experiments consisted of generating disinfection plans for Floatbot, Armbot, and Towerbot under a strict irradiation time limit of 30 minutes, as well as under a 100-hour time budget to the evaluate asymptotic disinfection performance of each design. We additionally evaluated placing Towerbot in the centroid of the room for the prescribed time budget to mimic the static status-quo.

% We then compared the total disinfection time of these 4 strategies: 
% \begin{itemize}
%     \item Executing an optimal disinfection plan for Floatbot
%     \item Executing an optimal disinfection plan for Armbot;
%     \item Executing an optimal disinfection plan for Towerbot
%     \item Placing Towerbot at the centroid of the room for as long as necessary to mimic the single-point status-quo.
% \end{itemize}

% We additionally performed the same experiments under a time constraint of 30 minutes in order to represent each strategy's efficiency under a strict time budget. 

\prettyref{fig: Robot Design Comparisons} illustrates that, as expected, robots with more degrees of freedom, like Armbot and Floatbot, disinfect more of the area, specially under tight time budgets and that, in accordance to \cite{Lindblad2019Ultraviolet-CNeeded}, the status-quo of static disinfection for tower-based roots fails to cover much of the surface, which is illustrated well in \prettyref{fig: single point 3D disnfection}. We note, however, that asymptotic performance is nearly identical among all mobile solutions.

Note, however, that the disinfection efficiency comes with tradeoff in total distance travelled, since Towerbot has the smallest trajectory length of all mobile solutions, whereas Armbot has the longest. 

This is likely due to two factors. First, distances in higher dimensions tend to be higher (3D vs 2D) and second, motion planning for Armbot involves many steps that are prone to suboptimality, such as vantage configuration selection given a desired lamp position and high-dimensional multi-query path planning, which is an active research area. Floatbot's trajectory length is a trivial lower bound to the Armbot's length. Jointly optimizing vantage configurations alongside a tour to minimize trajectory length is left to future research. 

Finally,\prettyref{fig:Smart 3D disnfection} shows a time-lapse of Armbot's disinfection trajectory.
% by Armbot  , where the disinfection trajectory of the UV lamp is highlighted in orange and the disinfection status of the room is color coded on a spectrum from red (0 fluence received) to solid green (received at least $\mu_{min} = 280 J/m^2$. 

\begin{figure}[htbp] % "[t!]" placement specifier just for this example
    \centering
    \includegraphics[width=0.95\linewidth]{figs/Robot Design Comparisons.pdf}
    \caption{Performance of robot designs disinfecting an infirmary} \label{fig: Robot Design Comparisons}
\end{figure}


% \begin{table}[htbp]
% \centering
% \begin{tabular}{ |l||c|c|c|c| } 

%  \hline \hline
%  \textbf{Method} & \textbf{Completion}  & \textbf{Coverage-1} & \textbf{Coverage-2}\\ & \textbf{time} & & \\
%  \hline
%  \textbf{Single} &  & & \\ 
%  \hline
%  \textbf{Towerbot} & 83.6 & & \\ 
%  \hline
%  \textbf{Ideal} & & & \\
%  \hline
%  \textbf{Armbot} & & & \\
%  \hline
% \end{tabular}
% \caption{Summary of 3D disinfection Experiments}
% \label{tab:3D experimental results}

% \end{table}

% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/2D example scene.pdf}
%     \caption{Example of the optimal 2D disinfection path on 2.5D scene} \label{fig: Example 2D trajectory}
% \end{figure}


    
%     \caption{Example of 2.5D disinfection of an empty square room. Vantage points are color-coded by the dwell time, and surface points are color-coded by the radiant exposure.  The single-point method underexposes the corners, so it takes 194\% more time than our method. } \label{fig: Empty Room disinfection}
%     \end{figure}


% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\linewidth]{figs/Complex Room disinfection Single.pdf}
%     \caption{Single Point Disinfection}
%     \end{subfigure}\hspace*{\fill}
%     \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\linewidth]{figs/Complex Room disinfection Multi.pdf}
%     \caption{Multipoint Disinfection} 
%     \end{subfigure}

    
%     \caption{Example of 2.5D disinfection of a room with randomly-generated obstacles. Both approaches were given the same time budget used by the multi-point disinfection to irradiate the room (400\,s). The single-point method only disinfects 20\% of the surfaces while our method disinfects the whole room.} \label{fig:2.5D disinfection of rooms}
%     \end{figure}
    
% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/single_tower_disinfection.png}
%     \caption{A stationary light source does not disinfect of the environment of Fig.~\ref{fig:Smart 3D disnfection} under the same 30 minutes budget nearly as well} \label{fig: single point 3D disnfection}
% \end{figure}


% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/histogram of time fractions.png}
%     \caption{Histogram of the fraction of time taken by movement during the disinfection of a set of 21 randomly generated 2.5D rooms} \label{fig: histogram of times}
% \end{figure}

% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/LP VS MILP.png}
%     \caption{Histogram of the extra time taken by our sequential approach when compared to the optimal solution} \label{fig: histogram of suboptimality}
% \end{figure}


\begin{figure*}[h!] % "[t!]" placement specifier just for this example
\setlength{\tabcolsep}{0.2px}
\begin{tabular}{cccc}
\includegraphics[width=.24\linewidth]{figs/7.5 minutes armbot.png}
\put(-110,-10){\small{Disinfection at 7.5 minutes}} &
\includegraphics[width=.24\linewidth]{figs/Armbot 15 minutes .png}
\put(-110,-10){\small{Disinfection at 15 minutes}} &
\includegraphics[width=.24\linewidth]{figs/22.5 armbot disinfection.png}
\put(-110,-10){\small{Disinfection at 22.5 minutes}} &
\includegraphics[width=.24\linewidth]{figs/30 minutes armbot.png}
\put(-110,-10){\small{Disinfection at 30 minutes}} 
\end{tabular}
\caption{Demonstration of optimized disinfection of a hospital room CAD model, with a time budget of 30 minutes. Red indicates no disinfection, green indicates complete disinfection. The light's path is shown in orange and visited dwell points are shown in yellow, while unvisited ones are shown in black} \label{fig:Smart 3D disnfection}
\end{figure*}

==> results_old2.tex <==
\section{\label{sec:results}Experiments \& Results}

\textcolor{I'm not seeing any absolute timing information.  Give times, scalability with \# of vantage configurations, \# of surfaces. }

\subsection{2.5D experiments}
\subsubsection{Comparison against single point}
We first evaluate our method in a baseline case of a 5m$\times$5m empty room - comparing single-point disinfection strategies with our proposed solution (The single point disinfection strategy consists in placing the disinfection light at the point that had maximum coverage over the obstacle space and allowing it to irradiate the surfaces for as long as necessary to fully disinfect its visible surfaces). \textcolor{red}{This discussion seems to have disappeared? Add this figure back, it's illustrative.}

We randomly generate 25 2.5D worlds with a number of geometric obstacles ranging from 7 to 19 obstacles (mean 13.7) and compare the maximum achievable coverage (i.e, the fraction of the surface area that received at least $\mu_{min}$ fluence) and time until full disinfection (time needed to guarantee $\mu_{min}$ fluence over all visible surfaces). In this scenario, we choose the sampling interval to be 0.25m. The results (\prettyref{fig: Single Point 2D Comparisons}) show that our proposed method consistently disinfects 100\% of the environment, whereas the optimal single vantage point could only disinfect, on average, 35\% of the environment's area, a difference clearly seen in \prettyref{fig: single point vs multi-point 2.5D}.  
\begin{figure}[H] % "[t!]" placement specifier just for this example
\vspace{-3px}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/Example of Optimally Placed Single point Disinfection.pdf}
\put(-120,88){\small{(a): Single Point Disinfection}}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}
\includegraphics[width=\linewidth]{figs/Ours 2D disinfection .pdf}
\put(-110,88){\small{(b): Multipoint Disinfection}} 
\end{subfigure}
\vspace{-3px}
\caption{Same room disinfected by the best single point (a) and by our method (b), where the trajectory is represented as a red line and each surface is colored according to the fluence it received.}
\label{fig: single point vs multi-point 2.5D}
\vspace{-10px}
\end{figure}


\subsubsection{Comparison against MILP formulation}
On a subset \textcolor{red}{what subset?} of the 2.5D rooms, we compare the two-stage scheme and the globally optimal MILP formulation described in our extended report~\cite{extended_report}. A point robot is limited to travel along a grid of waypoints at 50cm resolution \textcolor{red}{what is the size of the grid, in terms of number of points in each dimension?} with $v_{max}=0.5$m/s. The results are illustrated in \prettyref{fig: MILP VS LP}.  Columns 1, 2, and 4 are normalized to the LP+TSP results.  Observe that the dwell times and disinfection times are nearly identical, with less than 2\% difference between the two-stage approach and the optimal solution. Dwell times take approximately $90$\% of total disinfection time, and furthermore the paths computed by the two-stage approach are nearly identical to the optimal solution.  Moreover, the two-stage approach is $30$ times faster than the optimal MILP solution, even in such a simplified setting.
\begin{figure}[tbp] % "[t!]" placement specifier just for this example
\centering
\includegraphics[trim=0 0 0 0,clip,width=0.9\linewidth]{figs/Single Point 2D comparisons.pdf}
\vspace{-3px}
\caption{Comparison between our method and single point strategy \textcolor{red}{Is this 2D?  Make the figure smaller and show the solution path.}} \label{fig: Single Point 2D Comparisons}
\vspace{-15px}
\end{figure}
\begin{figure}[H] % "[t!]" placement specifier just for this example
\centering
\includegraphics[trim=0 0 0 0,clip,width=0.9\linewidth]{figs/MILP and LP comparisons.pdf}
\caption{Comparison between two-stage approach and the optimal MILP. Times normalized w.r.t. LP+TSP times for contrast.} \label{fig: MILP VS LP}
\end{figure}

% When compared to the optimal MILP formulation of the trajectory optimization problem, our proposed solution,at least for the gridding resolutions used, did not manifest a remarked loss of optimality, taking, on average, only 2.7\% longer to completely disinfect the 2.5D environments. In addition, our initial hypothesis that the majority of the disinfection time would be dwell time was confirmed since, in both algorithms, the time to move between the vantage points represented fewer than 10\% of the total disinfection time. In addition, our method was remarkably faster than the true optimal solution, which took, on average, 31.5 times longer to compute . \textcolor{red}{missing measure of spread - asked Ramya for data}


\subsection{3D experiments}
Our 3D tests were performed in a hospital infirmary's CAD model\footnote{https://grabcad.com/library/hospital-ward-2-2} (\prettyref{fig:Smart 3D disnfection}), modified for cohesion and scaling \textcolor{red}{What is cohesion? What size did you scale it to?}. Our experiments consist of generating disinfection plans for Floatbot, Armbot, and Towerbot \textcolor{red}{You need to describe these! You took the description out} under an irradiation time limit of $T_{max}=30$ minutes \textcolor{red}{Include a figure illustrating each model}.
\begin{figure}[tbp] % "[t!]" placement specifier just for this example
\centering
\includegraphics[width=0.95\linewidth]{figs/Robot Design Comparisons.pdf}
\caption{Performance of robot designs disinfecting an infirmary. \textcolor{red}{For Figs 5-7, shrink the figure size while keeping the text at the same size. There's no reason for them to be so big}} \label{fig: Robot Design Comparisons}
\end{figure}
In the vantage point selection step, our sampling interval is 0.25\,m. \textcolor{red}{What are the max speeds of the robots and the wattage of the lamp?}

We also compare with the strategy of placing Towerbot in the center of the room for the prescribed time budget to mimic the static status-quo. \prettyref{fig: Robot Design Comparisons} illustrates that robots with more degrees of freedom, like Armbot and Floatbot, disinfect more of the area, specially under tight time budgets and that, in accordance to \cite{Lindblad2019Ultraviolet-CNeeded}, the status-quo of static disinfection for Towerbot fails to cover much of the surface, as illustrated in \prettyref{fig: single point 3D disnfection}. The asymptotic performance is nearly identical among all mobile solutions, whereas the disinfection efficiency comes with a tradeoff in total distance travelled, among which Towerbot has the smallest trajectory length and Armbot has the longest. This is presumably due to two factors. First, distances in higher dimensions tend to be higher (3D vs 2D) and, second, motion planning for Armbot involves many steps that are prone to sub-optimality, such as vantage configuration selection given a desired lamp position and high-dimensional multi-query path planning. Floatbot's trajectory length is a trivial lower bound to the Armbot's length.

% \begin{table}[htbp]
% \centering
% \begin{tabular}{ |l||c|c|c|c| } 

%  \hline \hline
%  \textbf{Method} & \textbf{Completion}  & \textbf{Coverage-1} & \textbf{Coverage-2}\\ & \textbf{time} & & \\
%  \hline
%  \textbf{Single} &  & & \\ 
%  \hline
%  \textbf{Towerbot} & 83.6 & & \\ 
%  \hline
%  \textbf{Ideal} & & & \\
%  \hline
%  \textbf{Armbot} & & & \\
%  \hline
% \end{tabular}
% \caption{Summary of 3D disinfection Experiments}
% \label{tab:3D experimental results}

% \end{table}

% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/2D example scene.pdf}
%     \caption{Example of the optimal 2D disinfection path on 2.5D scene} \label{fig: Example 2D trajectory}
% \end{figure}


    
%     \caption{Example of 2.5D disinfection of an empty square room. Vantage points are color-coded by the dwell time, and surface points are color-coded by the radiant exposure.  The single-point method underexposes the corners, so it takes 194\% more time than our method. } \label{fig: Empty Room disinfection}
%     \end{figure}


% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\linewidth]{figs/Complex Room disinfection Single.pdf}
%     \caption{Single Point Disinfection}
%     \end{subfigure}\hspace*{\fill}
%     \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\linewidth]{figs/Complex Room disinfection Multi.pdf}
%     \caption{Multipoint Disinfection} 
%     \end{subfigure}

    
%     \caption{Example of 2.5D disinfection of a room with randomly-generated obstacles. Both approaches were given the same time budget used by the multi-point disinfection to irradiate the room (400\,s). The single-point method only disinfects 20\% of the surfaces while our method disinfects the whole room.} \label{fig:2.5D disinfection of rooms}
%     \end{figure}
    
% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/single_tower_disinfection.png}
%     \caption{A stationary light source does not disinfect of the environment of Fig.~\ref{fig:Smart 3D disnfection} under the same 30 minutes budget nearly as well} \label{fig: single point 3D disnfection}
% \end{figure}


% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/histogram of time fractions.png}
%     \caption{Histogram of the fraction of time taken by movement during the disinfection of a set of 21 randomly generated 2.5D rooms} \label{fig: histogram of times}
% \end{figure}

% \begin{figure}[htbp] % "[t!]" placement specifier just for this example
%     \centering
%     \includegraphics[width=0.96\linewidth]{figs/LP VS MILP.png}
%     \caption{Histogram of the extra time taken by our sequential approach when compared to the optimal solution} \label{fig: histogram of suboptimality}
% \end{figure}


\begin{figure*}[tbp] % "[t!]" placement specifier just for this example
\centering
\setlength{\tabcolsep}{0.2px}
\begin{tabular}{cc}
\includegraphics[width=.45\linewidth]{figs/7.5 minutes armbot.png}
\put(-220,5){\small{7.5\,min}} &
\includegraphics[width=.45\linewidth]{figs/Armbot 15 minutes .png}
\put(-220,5){\small{15\,min}}\\
\includegraphics[width=.45\linewidth]{figs/22.5 armbot disinfection.png}
\put(-220,5){\small{22.5\,min}} &
\includegraphics[width=.45\linewidth]{figs/30 minutes armbot.png}
\put(-220,5){\small{30\,min}} 
\end{tabular}
\vspace{-7px}
\caption{Time lapse of Armbot's disinfection progress for an infirmary within a time budget of 30 minutes. \textcolor{red}{Maybe draw the path of the light source.  Highlight the light?  The figures can be drawn smaller as well.} } \label{fig:Smart 3D disnfection}
\vspace{-12px}
\end{figure*}
